Uniform Approximations for Randomized Hadamard Transforms with Applications

Randomized Hadamard Transforms (RHTs) have emerged as a computationally efficient alternative to the use of dense unstructured random matrices across a range of domains in computer science and machine learning. For several applications such as dimensionality reduction and compressed sensing, the theoretical guarantees for methods based on RHTs are comparable to approaches using dense random matrices with i.i.d.\ entries. However, several such applications are in the low-dimensional regime where the number of rows sampled from the matrix is rather small. Prior arguments are not applicable to the high-dimensional regime often found in machine learning applications like kernel approximation. Given an ensemble of RHTs with Gaussian diagonals, $\{M^i\}_{i = 1}^m$, and any $1$-Lipschitz function, $f: \mathbb{R} \to \mathbb{R}$, we prove that the average of $f$ over the entries of $\{M^i v\}_{i = 1}^m$ converges to its expectation uniformly over $\| v \| \leq 1$ at a rate comparable to that obtained from using truly Gaussian matrices. We use our inequality to then derive improved guarantees for two applications in the high-dimensional regime: 1) kernel approximation and 2) distance estimation. For kernel approximation, we prove the first \emph{uniform} approximation guarantees for random features constructed through RHTs lending theoretical justification to their empirical success while for distance estimation, our convergence result implies data structures with improved runtime guarantees over previous work by the authors. We believe our general inequality is likely to find use in other applications.

==> content/algorithms.tex <==
% \section{Algorithms}
% \label{sec:alg}

% In this section, we formally describe our algorithms for kernel approximation and distance estimation through the use of structured orthogonal matrices. 

% \subsection{Kernel Approximation}
% \label{ssec:kern_approx_alg}

% \begin{algorithm}[H]
%     \begin{algorithmic}
%         \State \textbf{Input: } Dimension $d$, Subset $\mc{W}$, Accuracy $\eps$, Failure Probability $\delta$
%         \State $m = \kernEmbedRep$ 
%         \State Let $\{D^i\}_{i = 1}^m$ be $m$ i.i.d random diagonal matrices with $D^{i}_{j,j} \overset{i.i.d}{\thicksim} \mc{N} (0, 1)$
%         \State Let $\{b^i\}_{i = 1}^m$ be $m$ i.i.d random vectors with $b^i_{j} \overset{i.i.d}{\thicksim} \unif ([0, 2\pi])$
%         \State \textbf{Return:} $\{(D^i, b^i)\}_{i = 1}^m$
%     \end{algorithmic}
%     \caption{\prodKernEmbedDS}
%     \label{alg:kern_ds}
%   \end{algorithm}
%   {}\jnote{for ``Diam'' the metric should be specified. Also, what is $\mathcal W$?}

% \begin{algorithm}[H]
%     \begin{algorithmic}
%         \State \textbf{Input: } Data structure $\{(D^i, b^i)\}_{i = 1}^m$, Data point $x \in \R^d$
%         \State Let $h^i (x) = \sqrt{2} \cdot \cos \lprp{\frac{1}{\gamma} \cdot H D^i x + b^i}$
%         \State \textbf{Return: } $h(x) = \frac{1}{\sqrt{md}} \cdot (h^1 (x), \dots, h^m (x))$
%     \end{algorithmic}
%     \caption{\prodKernEmbed}
%     \label{alg:kern_embed}
% \end{algorithm}

==> content/cdf_proof.tex <==
\section{Proof of Uniform CDF Concentration}
\label{sec:cdf_proof}

% \jnote{Some of the lemma proofs should go in the appendix, so we can get to the kernel section in the first 10 pages} 
In this section, we formally prove \cref{thm:cdf_conc} by expanding on the outline presented in \cref{sec:proof_overview}. We begin by defining the class of functions for which our concentration properties will hold:
\begin{align*}
    G(s) &\coloneqq 
    \begin{cases}
        1, &\text{if } s \leq 0 \\
        1 - x, &\text{if } 0 < s < 1 \\
        0, &\text{otherwise}
    \end{cases}\\
    \forall S \subseteq [d]: V_S &\coloneqq \bigcup_{j = 1}^m \lbrb{D^j_{i, i}}_{i \in S} \\
    \forall S \subset [d], t \in \R, z \in \R^d, \eta \in \R_+ : F_{S, t, \eta} (z) &\coloneqq \frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d G\lprp{\eta (\wt{h}_{j,k}(z_{S}) - t)} \\
    \forall S, T \subseteq [d], t \in \R, z \in \R^d, \eta \in \R_+ : \wt{F}_{S, T, t, \eta} (z) &\coloneqq \mb{E}\lsrs{F_{S \cup T, t, \eta} (z) \mid V_T} \tag{CDF-NOT} \label{eq:cdf_not}
\end{align*}
To help define the nets used in our argument, we introduce the following notation and define:
\begin{gather*}
    \eta \coloneqq \cdfSlope, \ \rho \coloneqq \cdfRes, \ \lambda \coloneqq \cdfWid, \ \nu \coloneqq \cdfAcc\\
    \forall S, T \subseteq [D]: \mc{G}_{S, T} \coloneqq \lbrb{z \in \R^d:  \norm{z} \leq 1,\ \forall i \notin S \cup T, z_i = 0,\ \forall i,j \in S, \frac{1}{2} \abs{z_j} \leq \abs{z_i} \leq 2 \abs{z_j}} \\
    r \coloneqq \cdfNSplits,\quad \zeta \coloneqq \cdfSens,\quad \mc{T} \coloneqq \lbrb{\pm i \cdot \zeta}_{i = 0}^{\lambda / \zeta} \tag{CDF-NET} \label{eq:cdf_net}
\end{gather*}
For all disjoint $S, T \subseteq [d]$ such that $\abs{T} \leq r \cdot \abs{S}$, let $\wt{\mc{G}}_{S, T}$ be an $\rho$-cover of $\mc{G}_{S,T}$. Note, we may assume that $\abs{\wt{\mc{G}}_{S,T}} \leq \lprp{\frac{10\lambda}{\rho}}^{(r + 1) \cdot \abs{S}}$ \cite[Corollary 4.2.13]{vershynin}. We now have the following claim:
\begin{claim}
    \label{clm:net_part_conc}
    We have:
    \begin{equation*}
        \forall t \in \mc{T}, S,T \text{ s.t } \abs{T} \leq r \cdot \abs{S}, T \cap S = \phi, z \in \wt{\mc{G}}_{S,T}: \abs{F_{S \cup T, t, \eta} (z) - \wt{F}_{S, T, t, \eta} (z)} \leq \nu
    \end{equation*}
    with probability at least $1 - \delta / 4$.
\end{claim}
\begin{proof}
    For the proof, we start by conditioning on $V_T$. Note that for all $i \in S$, we must have:
    \begin{equation*}
        \abs{z_i} \leq \frac{2}{\sqrt{\abs{S}}}.
    \end{equation*}
    Let $V^1_S$ and $V^2_S$ be two distinct settings of the random variables $V_S$ and let $F^1_{S, t, \eta} (x), F^2_{S, t, \eta} (x)$ be the values of $F_{S, t, \eta}$ computed by setting the variables in $V_S$ to $V^1_S$ and $V^2_S$ respectively fixing all the rest to be the same. Similarly, let $\wt{h}^1(\cdot), \wt{h}^2(\cdot)$ denote the vectors $\wt{h}$ computed with the corresponding settings of $V_S$ and $D^{j,1}, D^{j,2}$ be the corresponding diagonal matrices for $j \in [m]$. Furthermore, observe that $G(\cdot)$ is an $\eta$-Lipschitz function. Hence, we have:
    \begin{align*}
        &\abs{F^1_{S, t, \eta} (z) - F^2_{S, t, \eta} (z)} \leq \frac{\eta}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \abs{\wt{h}^1_{j,k} (z) - \wt{h}^2_{j,k} (z)} \leq \frac{\eta}{\sqrt{md}} \cdot \sqrt{\sum_{j = 1}^m \sum_{k = 1}^d (\wt{h}^1_{j,k} (z) - \wt{h}^2_{j,k} (z))^2} \\
        &\leq \frac{\eta}{\sqrt{md}} \cdot 
        \norm*{
            \begin{bmatrix}
                H (D^{1, 1} - D^{1, 2}) z \\
                H (D^{2, 1} - D^{2, 2}) z \\
                \vdots \\
                H (D^{m, 1} - D^{m, 2}) z
            \end{bmatrix}
        } = \frac{\eta}{\sqrt{md}} \cdot 
        \norm*{
            \begin{bmatrix}
                H & 0 & \dots & 0\\
                0 & H & \dots & 0\\
                \vdots & \vdots & \ddots & \vdots\\
                0 & 0 & \dots & H
            \end{bmatrix} \cdot 
            \begin{bmatrix}
                (D^{1,1} - D^{1,2}) z \\
                (D^{2,1} - D^{2,2}) z \\
                \vdots \\
                (D^{m,1} - D^{m,2}) z
            \end{bmatrix}} \\
        &\leq \frac{\eta}{\sqrt{m}} \cdot 
        \norm*{
            \begin{bmatrix}
                (D^{1,1} - D^{1,2}) z \\
                (D^{2,1} - D^{2,2}) z \\
                \vdots \\
                (D^{m,1} - D^{m,2}) z
            \end{bmatrix}
        } = 
        \frac{\eta}{\sqrt{m}} \cdot 
        \norm*{
            \begin{bmatrix}
                \Diag (z) \diag(D^{1,1} - D^{1,2}) \\
                \Diag (z) \diag(D^{2,1} - D^{2,2}) \\
                \vdots \\
                \Diag (z) \diag(D^{m,1} - D^{m,2})
            \end{bmatrix}
        } \leq 2 \cdot \frac{\eta}{\sqrt{m}} \cdot \frac{1}{\sqrt{\abs{S}}} \cdot \norm{V^1_S - V^2_S}
    \end{align*}
    Therefore, $F_{S, t, \eta}$ is a $\frac{2 \eta}{\sqrt{m \abs{S}}}$-Lipschitz function of $V_S$. From our conditioning of $T$, we have by \cref{thm:tsirelson}:
    \begin{equation*}
        \P \lbrb{\abs{F_{S, t, \eta} (z) - \wt{F}_{S, T, t, \eta} (z)} \leq \nu} \geq 1 - \frac{\delta}{32 \cdot (10 / \rho)^{(r + 1)\cdot \abs{S}}\cdot (d + 1)^{(r + 1) \cdot \abs{S}} \cdot \abs{\mc{T}} \cdot d^2}.
    \end{equation*}
    The claim now follows from a union bound over all possible $S, T$ satisfying the constraints.
\end{proof}

% We now condition on the conclusion of the \cref{clm:net_part_conc} and prove a spectral norm bound on the linear transformation $\wt{h}$ in the following claim:
% \begin{claim}
%     \label{clm:h_spec_bnd}
%     We have:
%     \begin{equation*}
%         \forall y, z \in \R^d: \norm{\wt{h} (y) - \wt{h} (z)} \leq \sqrt{2md} \cdot \norm{x - y}
%     \end{equation*}
%     with probability at least $1 - \delta / 4$.
% \end{claim}
% \begin{proof}
%     We have
%     \begin{equation*}
%         \wt{h} (z) = 
%         \begin{bmatrix}
%             HD^1 \\
%             HD^2 \\
%             \vdots \\
%             HD^m
%         \end{bmatrix} z \text{ and }
%         \begin{bmatrix}
%             D^1 H^\top & D^2 H^\top & \dots & D^1 H^\top
%         \end{bmatrix}
%         \cdot
%         \begin{bmatrix}
%             HD^1 \\
%             HD^2 \\
%             \vdots \\
%             HD^m
%         \end{bmatrix}
%         = d \sum_{j = 1}^m (D^j)^2 
%         \preccurlyeq 2md \cdot I
%     \end{equation*}
%     with probabilty at least $1 - \delta / 4$. Conditioning on the above event, we get:
%     \begin{equation*}
%         \forall y,z \in \R^d: \norm*{\wt{h} (y) - \wt{h} (z)} \leq \sqrt{2md} \cdot \norm{y - z}.
%     \end{equation*}    
% \end{proof}
With \cref{clm:net_part_conc,lem:h_spec_bnd}, we now extend the conclusion of \cref{clm:net_part_conc} to all $z \in \mc{G}_{S,T}$.
\begin{claim}
    \label{clm:part_conc}
    Conditioning on the conclusions of \cref{clm:net_part_conc,lem:h_spec_bnd}, we have:
    \begin{equation*}
        \forall t \in \mc{T}, S,T \text{ s.t } \abs{T} \leq r \cdot \abs{S}, z \in \mc{G}_{S,T},\ T \cap S = \phi : \abs{F_{S \cup T, t, \eta} (z) - \wt{F}_{S, T, t, \eta} (z)} \leq 2\nu.
    \end{equation*}
\end{claim}
\begin{proof}
    We condition on \cref{clm:net_part_conc,lem:h_spec_bnd}. Let $z \in \mc{G}_{S,T}, t \in \mc{T}$ for $S,T$ satisfying the constraints and $\wt{z} = \argmin_{u \in  \wt{\mc{G}}_{S,T}} \norm{z - u}$. Note that $\norm{z - \wt{z}} \leq \rho$. We simply show that $F_{S \cup T, t, \eta}, \wt{F}_{S, T, t, \eta}$ are close to their corresponding values for $\wt{z}$. For the first, we have:
    \begin{align*}
        \abs{F_{S \cup T, t, \eta}(z) - F_{S \cup T, t, \eta}(\wt{z})} &= \frac{1}{md} \cdot \abs*{\sum_{j = 1}^m \sum_{k = 1}^d G(\eta (\wt{h}_{j, k} (z_{S \cup T}) - t)) - G(\eta (\wt{h}_{j, k} (\wt{z}_{S \cup T}) - t)} \\
        &\leq \frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \abs*{G(\eta (\wt{h}_{j, k} (z_{S \cup T}) - t)) - G(\eta (\wt{h}_{j, k} (\wt{z}_{S \cup T}) - t)} \\
        &\leq \frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \eta \abs*{\wt{h}_{j,k}(z_{S \cup T}) - \wt{h}_{j,k}(\wt{z}_{S \cup T})} \\
        &\leq \frac{\eta}{md} \cdot \sqrt{md} \cdot \sqrt{\sum_{j = 1}^m \sum_{k = 1}^d \lprp{\wt{h}_{j, k}(z_{S \cup T}) - \wt{h}_{j, k}(\wt{z}_{S \cup T})}^2} \\
        &\leq \frac{\eta}{\sqrt{md}} \cdot \sqrt{2md} \cdot \rho \leq \frac{\nu}{4}
    \end{align*}
    concluding the proof for the first term. For the second term, we proceed as follows:
    \begin{align*}
        \abs*{\wt{F}_{S, T, t, \eta} (z) - \wt{F}_{S, T, t, \eta} (\wt{z})} &= \abs*{\E \lsrs{F_{S \cup T, t, \eta}(z) - F_{S \cup T, t, \eta} (\wt{z})\mid V_T}} \\
        &\leq \frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \mb{E} \lsrs{\abs{G(\eta (\wt{h}_{j, k} (z_{S \cup T}) - t)) - G(\eta (\wt{h}_{j, k} (\wt{z}_{S \cup T}) - t))} \mid V_T} \\
        &\leq \frac{\eta}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \E \lsrs{\abs{\wt{h}_{j,k} (z_{S \cup T}) - \wt{h}_{j,k} (\wt{z}_{S \cup T})} \mid V_T} \\
        &\leq \frac{\eta}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \E \lsrs{\abs{\wt{h}_{j,k} (z_{S}) - \wt{h}_{j,k} (\wt{z}_{S})} + \abs{\wt{h}_{j,k} (z_{T}) - \wt{h}_{j,k} (\wt{z}_{T})}\mid V_T} \\
        &= \frac{\eta}{md} \cdot \lprp{\sum_{j = 1}^m \sum_{k = 1}^d \rho \cdot \E_{g \thicksim \mc{N}(0, 1)} \lsrs{\abs{g}} + \abs{\wt{h}_{j, k} (z_T) - \wt{h}_{j, k} (\wt{z}_T)}} \\
        &\leq \rho \eta \E_{g \thicksim \mc{N}(0, 1)} \lsrs{\abs{g}} + \frac{\eta}{md} \cdot \sqrt{md} \cdot \sqrt{\sum_{j = 1}^m \sum_{k = 1}^d (\wt{h}_{j, k} (z_T) - \wt{h}_{j, k}(\wt{z}_T))^2} \\
        &\leq \frac{\nu}{4} + \frac{\eta}{\sqrt{md}} \cdot \sqrt{2md} \cdot \rho \leq \frac{\nu}{2}.
    \end{align*}
    The previous two bounds along with the conclusion of \cref{clm:net_part_conc} yield the claim.
\end{proof}

From now on, we condition on the conclusions of \cref{lem:h_spec_bnd,clm:part_conc}. Let $z \in \R^d$ with $\norm{z} = 1$. We decompose the coordinates of $z$ into disjoint sets defined as follows:
\begin{equation*}
    \tau^* \coloneqq \max_{k \in [d]} \abs{z_k}, \quad \forall l \in [r]: S_l \coloneqq \lbrb{k: \frac{1}{2^l} \cdot \tau^* < \abs{z_k} \leq \frac{1}{2^{l - 1}} \cdot \tau^*}.
\end{equation*}
Let $S_{(1)}, \dots, S_{(r)}$ be an ordering of the $S_l$ such that $\abs{S_{(i)}} \leq \abs{S_{(i + 1)}}$ for all $i \in [r - 1]$ and define the sets $S^l$:
\begin{equation*}
    \forall l \in [r]: S^l \coloneqq \cup_{q = 1}^l S_{(q)} \text{ and } T \coloneqq [d] \setminus S^r.
\end{equation*}

We now show that as far as the functions $F$ are concerned, $z$ is well approximated by $z_{S^r}$.
\begin{claim}
    \label{clm:z_zsr}
    We have for all $t \in \R$:
    \begin{gather*}
        \abs*{\E \lsrs{F_{[d], t, \eta} (z) - F_{S^r, t, \eta} (z_{S^r})}} \leq \frac{\nu}{4}\\
        \abs*{F_{[d], t, \eta} (z) - F_{S^r, t, \eta} (z_{S^r})} \leq \frac{\nu}{4}.
    \end{gather*}
\end{claim}
\begin{proof}
    We make the following simple observation:
    \begin{equation}
        \label{eq:part_rem_bnd}
        \norm{z_{T}} \leq \sqrt{d} \cdot \frac{1}{2^r} \leq \rho.
    \end{equation}
    From \cref{eq:part_rem_bnd}, we have:
    \begin{align*}
        \abs*{\E \lsrs{F_{[d], t, \eta} (z) - F_{S^r, t, \eta} (z_{S^r})}} &= \abs*{\E \lsrs{F_{[d], t, \eta} (z) - F_{[d], t, \eta} (z_{S^r})}} \\
        &\leq \frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \E \lsrs{\abs*{G(\eta (\wt{h}_{j,k} (z) - t)) - G(\eta (\wt{h}_{j,k} (z_{S^r}) - t))}} \\
        &\leq \frac{\eta}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \E \lsrs{\abs*{\wt{h}_{j,k} (z) - \wt{h}_{j,k} (z_{S^r})}} \leq \eta \cdot \rho \cdot \E_{g \thicksim \mc{N}(0, 1)} [\abs{g}] \leq \frac{\nu}{4}.
    \end{align*}
    Similarly, we have:
    \begin{align*}
        \abs*{F_{[d], t, \eta} (z) - F_{S^r, t, \eta} (z_{S^r})} &= \abs*{F_{[d], t, \eta} (z) - F_{[d], t, \eta} (z_{S^r})} \\
        &\leq \frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \abs*{G(\eta (\wt{h}_{j,k} (z) - t)) - G(\eta (\wt{h}_{j,k} (z_{S^r}) - t))} \\
        &\leq \frac{\eta}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \abs*{\wt{h}_{j,k} (z) - \wt{h}_{j,k} (z_{S^r})} \leq \frac{\eta}{md} \cdot \sqrt{md} \cdot \sqrt{\sum_{j = 1}^m \sum_{k = 1}^d (\wt{h}_{j,k} (z) - \wt{h}_{j,k} (z_{S^r}))^2} \\
        &\leq \frac{\eta}{\sqrt{md}} \cdot \sqrt{2md} \cdot \rho \leq \frac{\nu}{4}
    \end{align*}
    concluding the proof of the claim.    
\end{proof}

In our final claim, we show that $F_{[d], t, \eta} (z_{S^r})$ is close to its expectation.
\begin{claim}
    \label{clm:approx_exp_close}
    We have:
    \begin{equation*}
        \forall l \in [r], t \in \R : \abs*{F_{S^l, t, \eta} (z_{S^l}) - \E \lsrs{F_{S^l, t, \eta} (z_{S^l})}} \leq 3l\nu.
    \end{equation*}
    and hence,
    \begin{equation*}
        \forall t \in \R : \abs*{F_{[d], t, \eta} (z) - \E \lsrs{F_{[d], t, \eta} (z)}} \leq 3(r + 1)\nu.
    \end{equation*}
\end{claim}
\begin{proof}
    We prove the claim inductively and start with the base case of the induction.
    \paragraph{Base case:} The base case is already established for all $t \in \mc{T}$. Now, note that $F_{S^1, t, \eta} (z_{S^1})$ and $\E [F_{S^1, t, \eta} (z_{S^1})]$ are monotonically increasing functions of $t$ and that $\norm*{z_{S^1}} \leq 1$. To extend to all $t \in \R$, we handle two cases for $t$ separately. 
    
    \noindent\textbf{Case 1:} For $t \geq \lambda$, we have:
    \begin{equation*}
        1 \geq \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \geq \mb{P}_{Y \thicksim \mc{N}(0, 1)} \lbrb{Y \leq \lambda} \geq 1 - \frac{\nu}{4}
    \end{equation*}
    and therefore, we get that:
    \begin{equation*}
        F_{S^1, t, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \leq 1 - \lprp{1 - \frac{\nu}{4}} \leq \frac{\nu}{4}
    \end{equation*}
    and
    \begin{equation*}
        F_{S^1, t, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \geq F_{S^1, \lambda, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \geq \lprp{1 - \frac{\nu}{4} - 2\nu} - 1 \geq - 3 \nu.
    \end{equation*}
    Similarly, we have for $t \leq -\lambda$:
    \begin{equation*}
        0 \leq \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \leq \mb{P}_{Y \thicksim \mc{N}(0, 1)} \lbrb{Y \leq -\lprp{\lambda - \frac{1}{\eta}}} \leq \frac{\nu}{4}.
    \end{equation*}
    Hence, we have:
    \begin{equation*}
        F_{S^1, t, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \geq 0 - \frac{\nu}{4} \geq -\frac{\nu}{4}
    \end{equation*}
    and
    \begin{equation*}
        F_{S^1, t, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \leq F_{S^1, -\lambda, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \leq \lprp{\frac{\nu}{4} + 2\nu} - 0 \leq 3\nu
    \end{equation*}
    establishing the base case in this case.

    \noindent\textbf{Case 2:} For $\abs{t} \leq \lambda$, there exist $t_1, t_2 \in \mc{T}$ with $\abs{t_1 - t_2} \leq \zeta$ and $t \in [t_1, t_2]$. Then, we have:
    \begin{align*}
        F_{S^1, t, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} &\leq F_{S^1, t_2, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \leq 2\nu + \E \lsrs{F_{S^1, t_2, \eta} (z_{S^1}) - F_{S^1, t, \eta} (z_{S^1})} \\
        &\leq 2\nu + \E \lsrs{\eta \cdot \abs{t_2 - t}} \leq 3\nu.
    \end{align*}
    Similarly, we have:
    \begin{align*}
        F_{S^1, t, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} &\geq F_{S^1, t_1, \eta} (z_{S^1}) - \E \lsrs{F_{S^1, t, \eta} (z_{S^1})} \geq -2\nu + \E \lsrs{F_{S^1, t_1, \eta} (z_{S^1}) - F_{S^1, t, \eta} (z_{S^1})} \\
        &\geq -2\nu - \E \lsrs{\eta \cdot \abs{t_1 - t}} \geq -3\nu
    \end{align*}
    establishing the base case in this setting as well.

    \paragraph{Inductive case:} For the induction step, we proceed similarly to the base case with one additional step. Assuming the induction up to $l = q$, we establish it for $l = q + 1$. First, we show that $\wt{F}_{S_{(q + 1)}, S^q, t, \eta} (z_{S^{q + 1}})$ is close to $\E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})}$ for all $t$. We proceed as follows:
    \begin{align*}
        &\abs*{\wt{F}_{S_{(q + 1)}, S^q, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta}(z_{S^{q + 1}})}} \\
        &= \abs*{\frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \E \lsrs{G (\eta (\wt{h}_{j, k}(z_{S^{q + 1}}) - t)) \mid V_{S^q}} - \E \lsrs{F_{S^{q + 1}, t, \eta}(z_{S^{q + 1}})}} \\
        &= \abs*{\frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \E_{g \thicksim \mc{N}(0, 1)} \lsrs{G (\eta (\norm{z_{S_{(q + 1)}}} \cdot g + \wt{h}_{j,k} (z_{S^{q}}) - t)) \mid V_{S^q}} - \E \lsrs{F_{S^{q + 1}, t, \eta}(z_{S^{q + 1}})}} \\
        &= \abs*{\frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \int_{-\infty}^\infty G(\eta (\norm{z_{S_{(q + 1)}}} \cdot y + \wt{h}_{j,k} (z_{S^q}) - t))\phi(y) dy - \E \lsrs{F_{S^{q + 1}, t, \eta}(z_{S^{q + 1}})}} \\
        &= \abs*{\int_{-\infty}^\infty F_{S^q, t - \norm*{z_{S_{(q + 1)}}} \cdot y, \eta} (z_{S^q}) \phi(y) dy - \E_{y_1, y_2 \thicksim \mc{N}(0, 1)} \lsrs{G(\eta (\norm{z_{S_{(q + 1)}}}\cdot y_1 + \norm{z_{S^q}} \cdot y_2 - t))}} \\
        &= \abs*{\int_{-\infty}^\infty F_{S^q, t - \norm*{z_{S_{(q + 1)}}} \cdot y, \eta} (z_{S^q}) \phi(y) dy - \int_{-\infty}^\infty \int_{-\infty}^\infty G (\eta (\norm{z_{S^q}} \cdot y_1 + \norm{z_{S_{(q + 1)}}} \cdot y_2 - t))\phi(y_1) \phi(y_2)dy_1 dy_2} \\
        &= \abs*{\int_{-\infty}^\infty \lprp{F_{S^q, t - \norm*{z_{S_{(q + 1)}}} \cdot y, \eta} (z_{S^q}) - \E \lsrs{F_{S^q, t - \norm*{z_{S_{(q + 1)}}} \cdot y, \eta} (z_{S^q})}} \phi(y) dy} \\
        &\leq \int_{-\infty}^\infty \abs*{F_{S^q, t - \norm*{z_{S_{(q + 1)}}} \cdot y, \eta} (z_{S^q}) - \E \lsrs{F_{S^q, t - \norm*{z_{S_{(q + 1)}}}, \eta} (z_{S^q})}} \phi(y) dy \leq 3q\nu.
    \end{align*}
    Now, as in the base case, we simply bound the deviations of $F$ from its expectation. From this, we get:
    \begin{equation*}
        \forall t \in \mc{T}: \abs*{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})}} \leq 2\nu + 3q\nu.
    \end{equation*}

    Similarly to the base case, the previous display establishes the inductive hypothesis for all $t \in \mc{T}$. We also have as before that $F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})$ and $\E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})}$ are monotonically increasing functions of $t$ and that $\norm{z_{S^{q + 1}}} \leq 1$. To extend to all $t \in \R$, we break into two cases as before:

    \noindent\textbf{Case 1:} For $\abs{t} \geq \lambda$, we have:
    \begin{equation*}
        1 \geq \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \geq \mb{P}_{Y \thicksim \mc{N}(0, 1)} \lbrb{Y \leq \lambda} \geq 1 - \frac{\nu}{4}
    \end{equation*}
    and therefore, we get that:
    \begin{equation*}
        F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \leq 1 - \lprp{1 - \frac{\nu}{4}} \leq \frac{\nu}{4}
    \end{equation*}
    and
    \begin{align*}
        F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} &\geq F_{S^{q + 1}, \lambda, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \\
        &\geq \lprp{1 - \frac{\nu}{4} - (3q + 2)\nu} - 1 \geq - 3(q + 1)\nu.
    \end{align*}
    Similarly, we have for $t \leq -\lambda$:
    \begin{equation*}
        0 \leq \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \leq \mb{P}_{Y \thicksim \mc{N}(0, 1)} \lbrb{Y \leq -\lprp{\lambda - \frac{1}{\eta}}} \leq \frac{\nu}{4}.
    \end{equation*}
    Hence, we have:
    \begin{equation*}
        F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \geq 0 - \frac{\nu}{4} \geq -\frac{\nu}{4}
    \end{equation*}
    and
    \begin{align*}
        F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} &\leq F_{S^{q + 1}, -\lambda, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \\
        &\leq \lprp{\frac{\nu}{4} + (3q + 2)\nu} - 0 \leq 3(q + 1)\nu
    \end{align*}
    establishing the result in this case.

    \noindent\textbf{Case 2:} For $\abs{t} \leq \lambda$, there exist $t_1, t_2 \in \mc{T}$ with $\abs{t_1 - t_2} \leq \zeta$ and $t \in [t_1, t_2]$. Then, we have:
    \begin{align*}
        F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} &\leq F_{S^{q + 1}, t_2, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \\
        &\leq (3q + 2)\nu + \E \lsrs{F_{S^{q + 1}, t_2, \eta} (z_{S^{q + 1}}) - F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \\
        &\leq (3q + 2)\nu + \E \lsrs{\eta \cdot \abs{t_2 - t}} \leq 3 (q + 1)\nu.
    \end{align*}
    Similarly, we have:
    \begin{align*}
        F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} &\geq F_{S^{q + 1}, t_1, \eta} (z_{S^{q + 1}}) - \E \lsrs{F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \\
        &\geq -(3q + 2)\nu + \E \lsrs{F_{S^{q + 1}, t_2, \eta} (z_{S^{q + 1}}) - F_{S^{q + 1}, t, \eta} (z_{S^{q + 1}})} \\
        &\geq -(3q + 2)\nu - \E \lsrs{\eta \cdot \abs{t_1 - t}} \geq -3(q + 1)\nu
    \end{align*}
    establishing the result in this setting as well. The final statement now follows from \cref{clm:z_zsr}.
\end{proof}

From \cref{clm:approx_exp_close}, we may conclude the proof of the theorem with the following manipulations:
\begin{align*}
    &\frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \bm{1} \lbrb{\wt{h}_{j,k} (z) \leq t} - \P_{Z \sim \mc{N}(0, 1)} (Z \leq t) \\
    &\leq F_{[d], t, \eta} (z) - \E \lsrs{F_{[d], t - \frac{1}{\eta}, \eta} (z)} \leq 3(r + 1)\nu + \E \lsrs{F_{[d], t, \eta} (z) - F_{[d], t - \frac{1}{\eta}, \eta} (z)} \\
    &\leq 3(r + 1)\nu + \P_{Y \thicksim \mc{N}(0, 1)} \lbrb{Y \leq t + \frac{1}{\eta}} - \P_{Y \thicksim \mc{N} (0, 1)} \lbrb{Y \leq t - \frac{1}{\eta}} \leq 3(r + 1)\nu + \frac{2}{\eta} \leq 3(r + 2) \nu.
\end{align*}
Similarly, we have for the other direction:
\begin{align*}
    &\frac{1}{md} \cdot \sum_{j = 1}^m \sum_{k = 1}^d \bm{1} \lbrb{\wt{h}_{j,k} (z) \leq t} - \P_{Z \sim \mc{N}(0, 1)} (Z \leq t) \\
    &\geq F_{[d], t - \frac{1}{\eta}, \eta} (z) - \E \lsrs{F_{[d], t, \eta} (z)} \geq - 3(r + 1)\nu - \E \lsrs{F_{[d], t, \eta} (z) - F_{[d], t - \frac{1}{\eta}, \eta} (z)} \\
    &\geq -3(r + 1)\nu - \P_{Y \thicksim \mc{N}(0, 1)} \lbrb{Y \leq t + \frac{1}{\eta}} + \P_{Y \thicksim \mc{N} (0, 1)} \lbrb{Y \leq t - \frac{1}{\eta}} \geq -3(r + 1)\nu - \frac{2}{\eta} \geq -3(r + 2) \nu.
\end{align*}
concluding the proof of the theorem.
\qed

==> content/notes.tex <==
\section{Notes and ToDos}

General ToDo:
\begin{enumerate}
    \item Write the algorithms - Easy for kernel approximation, some minor inconveniences for distance estimation
    \item Write proofs:
    \begin{enumerate}
        \item Easy for distance estimation - basic truncation function is Lipschitz. So, the proof should follow from standard techniques Lipschitz concentration of gaussian results.
        \item A little more involved for kernel approximation - the order of the union bounds will depend on the precise grouping of the terms involved (the number of terms in each grouping of the coordinates).
    \end{enumerate}
\end{enumerate}

